Cylindrical coordinates for LiDAR point cloud compression

We present an efficient voxelization method to encode the geometry and attributes of 3D point clouds obtained from autonomous vehicles. Due to the circular scanning trajectory of sensors, the geometry of LiDAR point clouds is inherently different from that of point clouds captured from RGBD cameras. Our method exploits these specific properties to representing points in cylindrical coordinates instead of conventional Cartesian coordinates. We demonstrate thatRegion Adaptive Hierarchical Transform (RAHT) can be extended to this setting, leading to attribute encoding based on a volumetric partition in cylindrical coordinates. Experimental results show that our proposed voxelization outperforms conventional approaches based on Cartesian coordinates for this type of data. We observe a significant improvement in attribute coding performance with 5-10%reduction in bitrate and octree representation with 35-45% reduction in bits.

==> voxelization_error.tex <==
\section{Voxelization error}
Let $x,y,z$ be the coordinates of a point in Cartesian coordinates. Let $\hat{x}, \hat{y},\hat{z}$ be the voxelized poin in cartesian coordinates, that is
\begin{align}
    \hat{x} &= Q\cdot round(x/Q) \\
    \hat{y} &= Q\cdot round(y/Q) \\
    \hat{z} &= Q\cdot round(z/Q).
\end{align}
When voxelizing in cartesian coordinates, we always use cubic voxel sizes. We can write the voxelization error as $\hat{x} = x + \epsilon_1$, $\hat{y} = y + \epsilon_2$ and $\hat{z} = z + \epsilon_3$, thus the total voxeliation error is
\begin{equation}
    (x - \hat{x})^2 +(y - \hat{y})^2 + (z - \hat{z})^2  = \epsilon_1^2 + \epsilon_2^2 + \epsilon_3^2.
\end{equation}
A typical assumption in analysis of quantization error is that $\epsilon_i$, are uniform with variance $Q^2/12$, and thus when using traditional voxelization, all axis are treated equally.

For cylindrical coordinates however we observe a different phenomenon. Assume the voxelization of $(r,\theta, h)$ are done as follows
\begin{align}
    \hat{r} &= Q_1\cdot round(r/Q_1) \\
    \hat{\theta} &= Q_2\cdot round(\theta/Q_2) \\
    \hat{h} &= Q_3\cdot round(h/Q_3).
\end{align}
Then the reconstruction formula in Cartesian coordinates is 
\begin{align}
    \hat{x} = \hat{r} cos(\hat{\theta}) \\
    \hat{y} = \hat{r} sin(\hat{\theta}) \\
    \hat{z} = \hat{h}.
\end{align}
Obviously, the error in the $z$ axis can be derived in the same manner as for the Cartesian voxelization. Now we will use the following notation for the voxeliation error in cylindrical coordinates

\begin{align}
    \hat{r} = r + \epsilon_1 \\
    \hat{\theta} = \theta + \epsilon_2.
\end{align}
Next we will derive a formula for the voxelization error. First note that
\begin{align}
    (\hat{x} - x)^2 + (\hat{y} - y)^2 = \hat{x}^2 + \hat{y}^2 + x^2 + y^2  -2\hat{x}x - 2 \hat{y} y.
\end{align}
Using the definition of $\hat{r}$ and $r$ as a function of their Cartesian counterparts we have that
\begin{align}
(\hat{x} - x)^2 + (\hat{y} - y)^2 &= \hat{r}^2 + r^2 -2r\hat{r}\left( cos(\theta)cos(\hat{\theta}) + sin(\theta) sin(\hat{\theta}) \right)\\
&= \hat{r}^2 + r^2 -2r\hat{r} cos(\epsilon_2).
\end{align}
Now we use the identity $\hat{r} = r + \epsilon_1$ and get
\begin{align}
 (\hat{x} - x)^2 + (\hat{y} - y)^2&= 2r^2 + 2r\epsilon_1 + \epsilon_1^2 - 2r^2 cos(\epsilon_2) - 2r\epsilon_1 cos(\epsilon_2) \\
 &= 2r^2 (1-cos(\epsilon_2)) + 2r\epsilon_1 (1-cos(\epsilon_2)) + \epsilon_1^2 \\
 & = 2r(r + \epsilon_1)(1-cos(\epsilon_2)) + \epsilon_1^2.
\end{align}
finally the total voxelization error is
\begin{align}
(\hat{x} - x)^2 + (\hat{y} - y)^2  + (\hat{z} - z)^2  = \epsilon_1^2 + 2r(r + \epsilon_1)(1-cos(\epsilon_2)) + \epsilon_3^2,  
\end{align}
where $\hat{h} = h + \epsilon_3$, and $\hat{z}=\hat{h}$, and $z=h$. The first and third terms correspond to errors in Radial and Height directions, and resemble those of Cartesian coordinates, in the sense that is independent of the magnitude of the signal along those directions. The second term contains interactions between angular and radial directions. The second term indicates that when the point (x,y,z) is close to the origin (r small), this term is negligible, and thus voxelization incurs in smaller errors. When the point is far away from the origin (r large), voxelization has larger error. Also note that we have the follow approximation due to Taylor expansion
\begin{equation}
    1-cos(\theta) = \frac{\theta^2}{2} + o(\theta^4).
\end{equation}
this implies that when the angular resolution is good enough ($\theta_2$ small), then 
\begin{equation}
 (\hat{x} - x)^2 + (\hat{y} - y)^2  + (\hat{z} - z)^2  \approx \epsilon_1^2 + r(r + \epsilon_1))\epsilon_2^2 + \epsilon_3^2   
\end{equation}
Assuming that $\epsilon_i$ are independent, zero mean, with variances $\sigma_i^2$ the expected error of point $(x,y,z)$ in cyclindrical coordinates is
\begin{equation}
    E[(\hat{x} - x)^2 + (\hat{y} - y)^2  + (\hat{z} - z)^2 ] \approx \sigma_1^2  + r^2 \sigma_2^2 + \sigma_3^2
\end{equation}
